Training Neural Networks Embedded in Dynamic Discrete Choice Models

We develop the first general-purpose estimator for infinite-horizon dynamic discrete choice models whose estimation problem, after pre-computation, is unencumbered by large systems of linear equations -- either imposed as constraints, or embedded in the objective function. Our unnested fixed point (UFXP) and optimal unnested fixed point (OUFXP) estimators exploit a dual representation of Bellman's equation to separate the utility parameters from the dynamic programming fixed point. We establish the consistency and asymptotic normality of UFXP and OUFXP, as well as the efficiency of the latter. Our estimators enable researchers to model utility functions non-parametrically via flexible neural-network approximations.

==> global.tex <==
%chunks of text
\newcommand{\qref}[1]{
	\section{}
	\begin{tcolorbox}[colback=gray!15]\small\setlength{\parindent}{3ex}
		#1
	\end{tcolorbox}
}

\newcommand{\qrefg}[1]{
	\begin{tcolorbox}[colback=gray!15]\small\setlength{\parindent}{3ex}
		#1
	\end{tcolorbox}
}

\newcommand{\qrefb}[1]{
	\begin{tcolorbox}[colback=blue!5!white, colframe=blue!60!black]\small\setlength{\parindent}{3ex}
		#1
	\end{tcolorbox}
}

\newcommand{\qrefw}[1]{
	\begin{tcolorbox}[colback=white, colframe=black]\small\setlength{\parindent}{3ex}
		#1
	\end{tcolorbox}
}

\newcommand{\qrefr}[1]{
	\begin{tcolorbox}[colback=red!5!white, colframe=red!60!black]\small\setlength{\parindent}{3ex}
		#1
	\end{tcolorbox}
}

%Long boxes that run across multiple pages
\newcommand{\qrefl}[1]{
	\section{}
	\begin{tcolorbox}[enhanced jigsaw,breakable,pad at break*=1mm]\small\setlength{\parindent}{3ex}
		#1
	\end{tcolorbox}
}

\newcommand{\qrefbl}[1]{
	\begin{tcolorbox}[enhanced jigsaw,breakable,pad at break*=1mm,colback=blue!5!white, colframe=blue!60!black]\small\setlength{\parindent}{3ex}
		#1
	\end{tcolorbox}
}

\newcommand{\qrefrl}[1]{
	\begin{tcolorbox}[enhanced jigsaw,breakable,pad at break*=1mm,colback=red!5!white, colframe=red!60!black]\small\setlength{\parindent}{3ex}
		#1
	\end{tcolorbox}
}

\newcommand{\hideText}[1]{}

\newcommand{\pref}[1]{\pageref{#1}}

\newcommand{\naive}{na\"{i}ve}
\newcommand{\Naive}{Na\"{i}ve}

%math expressions
\newcommand{\indicator}[1]{\mathbbm{1}\{#1\}}
\newcommand{\indicatorbig}[1]{\mathbbm{1}\big\{#1\big\}}
\newcommand{\indicatorBig}[1]{\mathbbm{1}\Big\{#1\Big\}}
\newcommand{\indicatorleft}[1]{\mathbbm{1}\left\{#1\right\}}
\newcommand{\iid}{$i.i.d.$}
\newcommand{\R}{\mathbbm{R}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\st}{such\ that}
\DeclareMathOperator*{\stt}{s.t.}
\DeclareMathOperator*{\colonBreak}{\,:\,}
\DeclareMathOperator*{\barBreak}{\,|\,}
\DeclareMathOperator*{\vertBreak}{\,|\,}
\DeclareMathOperator*{\E}{E}
\DeclareMathOperator*{\var}{Var}
\DeclareMathOperator*{\cov}{Cov}
\DeclareMathOperator*{\std}{StDv}
\DeclareMathOperator*{\diag}{diag}
\DeclareMathOperator*{\Tr}{Tr}
\DeclareMathOperator*{\vect}{vec}
\DeclareMathOperator*{\spn}{span}
\DeclareMathOperator{\sign}{sign}

%table spacing
\newcommand\up{\rule{0pt}{2.6ex}}
\newcommand\down{\rule[-1.2ex]{0pt}{0pt}}
\def\VSpace{1.0ex}

%colors
\definecolor{deepBlue}{rgb}{0.2, .2, .7}
\definecolor{LightGrey}{rgb}{0.9, .9, .9}
\newcommand{\red}[1]{{\color{red} #1}}
\newcommand{\blue}[1]{{\color{blue} #1}}

%this appends chapter-specific tags to each label
\newcommand{\cBreak}{}
\newcommand{\labelc}[1]{\label{\cBreak c\arabic{chapter}:#1}}
\newcommand{\refc}[1]{\ref{\cBreak c\arabic{chapter}:#1}}
\newcommand{\eqrefc}[1]{\eqref{\cBreak c\arabic{chapter}:#1}}
\newcommand{\appendixc}{\appendix\renewcommand{\cBreak}{A:}}

%lists that indent at new paragraphs, and have less space between bullets
\newenvironment{myitm}{%
	\edef\backupindent{\the\parindent}%
	\itemize\itemsep0em
	\setlength{\parindent}{\backupindent}%
}{\enditemize}

\newenvironment{myenm}{%
	\edef\backupindent{\the\parindent}%
	\enumerate\itemsep0em
	\setlength{\parindent}{\backupindent}%
}{\endenumerate}

%columns
%\newcolumntype{t}{D{.}{.}{3.5}}
\newcolumntype{g}{D{.}{.}{3}}



%references
\newcommand{\sref}[1]{\S\ref{#1}}
\newcommand{\cites}[1]{\citeauthor{#1}'s \citeyearpar{#1}}
\newcommand{\citess}[2]{\citeauthor{#1}'s \citeyearpar{#1, #2}}
\newcommand{\citeauthors}[1]{\citeauthor{#1}'s}
\newcommand{\citets}[2]{\citeauthor{#2}'s \citeyearpar[#1]{#2}}

%keywords
\newcommand{\setKeywords}[1]{
	~ \li \noindent\emph{Keywords}: #1
}
\newcommand{\subjectClassification}[1]{
	~ \li \noindent\emph{Subject Classification}: #1
}

%make line
\newcommand{\li}{\\~\\}

%itemize
\newcommand{\itm}[1]{
	\begin{itemize}
		#1
	\end{itemize}
}
\newcommand{\enm}[1]{
	\begin{enumerate}
		#1
	\end{enumerate}
}


%right arrow
\newcommand{\ra}{$\rightarrow$\ }
\newcommand{\Ra}{$\Rightarrow$\ }

%sim
\newcommand{\s}{$\sim$\ }

%boldsymbol
\newcommand{\bs}[1]{\boldsymbol{#1}}

%Longpage mode
\ifdefined\largePage
\geometry{paperwidth=500mm, paperheight=16383pt, left=40pt, top=40pt, textwidth=280pt, marginparsep=20pt, marginparwidth=100pt, textheight=16263pt, footskip=40pt}
\setcounter{totalnumber}{100}
\fi

%Set handout mode
\newcommand{\setHandouts}{
	\iftoggle{Handout}{
		\setbeameroption{hide notes}
	}{
		\setbeameroption{show notes on second screen=right}
	}	
}

%If it's in handout mode show #1 otherwise show #2
\newcommand{\hif}[2]{
	\iftoggle{Handout}{
		#1
	}{
		#2
	}
}

%Homework solution answer
\newcommand{\aif}[1]{
	\iftoggle{Answers}{
		\begin{tcolorbox}[enhanced jigsaw,breakable,pad at break*=1mm,colback=blue!5!white,
			title= Answer, colframe=blue!60!black]\small\setlength{\parindent}{3ex}
			#1
		\end{tcolorbox}
	}
}

\newcommand{\discussThis}{
	\begin{center}
		\textbf{**********************DISCUSS THIS **********************}
	\end{center}
}
%teaching title
\newcommand{\teachingTitle}[2]{
	\addtobeamertemplate{block begin}{\setlength\abovedisplayskip{0pt}}
	
	\title{#1}
	\author[Bray]{Robert L. Bray}
	\date{}
	\institute[Kellogg School of Management]{Kellogg School of Management}
	\AtBeginSection[]{\frame{{#1}\tableofcontents[currentsection,currentsubsection]}}
	\AtBeginSubsection[]{\frame{{#1}\tableofcontents[currentsection,currentsubsection]}
		\AtBeginSubsubsection[]{\frame{{#1}\tableofcontents[currentsection,currentsubsection]}}
	}
	
	\frame{
		\titlepage
		\nt{
			\begin{center}\LARGE \textcolor{red}{Module Notes} \end{center}
			#2
		}
	}
	
	\frame{{#1}
		\tableofcontents{}
	}
}

%Use the "visible" function only in presentation mode. #1 is the control given to visible, and #2 is the text
\newcommand{\hvis}[2]{\hif{#2}{\visible<#1>{#2}}}

%Use the "uncover" function only in presentation mode. #1 is the control given to uncover, and #2 is the text
\newcommand{\hunc}[2]{\hif{#2}{\uncover<#1>{#2}}}

%When you want onslides to be different in handout and presentation mode
\newcommand{\honslide}[2]{\hif{\onslide<#1>}{\onslide<#2>}}

%If there's an overprint in your notes, but not in your slides, you need this for your notes to show up
\newcommand{\loadNotes}{\hif{}{\visible<2>{}}}

%note that disapears in handout mode
\newcommand{\nt}[1]{\hif{}{\note{#1}}}

%bold
\newcommand{\bo}[1]{\textbf{#1}}

%bold
\newcommand{\emphbf}[1]{\emph{\textbf{#1}}}

%alert
\newcommand{\al}[1]{\alert{#1}}

%Next slide prompt
\newcommand{\ns}{\al{\bo{Next slide}}}
\newcommand{\ds}{\textcolor{green}{\bo{Student discussion}}}


%Hard prompt
\newcommand{\hard}{\al{\bo{Hard:}} }

%Week in math mode
\newcommand{\wk}{\text{wk}}

%Create a color box: cb{color}{width}
\newcommand{\cb}[2]{\colorbox{#1}{\strut\parbox{#2}{~}}}

%Grey color box:
\newcommand{\gb}[1]{\cb{LightGrey}{#1}}

%nonumber
\newcommand{\n}{\nonumber\\}
\newcommand{\no}{\nonumber}

%and and where

\newcommand{\aq}{\text{and}\quad}
\newcommand{\wq}{\text{where}\quad}
\newcommand{\wiq}{\text{which implies}\quad}
\newcommand{\fq}{\text{for}\quad}

%widehat
\newcommand{\wh}[1]{\widehat{#1}}

%big space
\newcommand{\q}[1]{
	\newcount\quadCount
	\quadCount=#1
	\loop
	\quad 
	\advance \quadCount -1
	\ifnum \quadCount>0	
	\repeat
}

\newcommand{\courier}[1]{{\fontfamily{pcr}\selectfont#1}}

%norms
\newcommand{\verti}[1]{
	{\vert #1 \vert}
}

\newcommand{\vertiiSingle}{\vert\kern-0.25ex\vert}

\newcommand{\vertii}[1]{
	{\vert\kern-0.25ex\vert #1 \vert\kern-0.25ex\vert}
}

\newcommand{\vertiii}[1]{
	{\vert\kern-0.25ex\vert\kern-0.25ex\vert #1 
		\vert\kern-0.25ex\vert\kern-0.25ex\vert}
}

\newcommand{\vertib}[1]{
	{\left\vert #1 \right\vert}
}
\newcommand{\vertiib}[1]{
	{\left\vert\kern-0.25ex\left\vert #1 
		\right\vert\kern-0.25ex\right\vert}
}
\newcommand{\vertiiib}[1]{
	{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
		\right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}
}
